Review of Hadron Structure Calculations on a Lattice

I present a review of the current status and the most recent achievements in lattice QCD calculations of hadron structure. First, I overview the status and systematic uncertainties of nucleon structure "benchmark" quantities that are well known from experiments and serve as a reference point for the validity of lattice QCD methods. Next, I discuss the current status of calculations of form factors of the nucleon and highlight some recent results for other hadrons that are important for understanding their internal dynamics. Wave functions of hadrons and their excitations may also be studied in lattice QCD, and I illustrate it with two recent examples of such calculations. Finally, I discuss in detail the state of calculations pertaining to the nucleon spin puzzle.

==> Makefile <==
all-tex		= syritsyn-lat13.tex
all-bib		= syritsyn-lat13.bib


text-dir	= text
figs-dir	= figs


ps-figs		= \


eps-figs	= \

pdf-figs	= \
		orig-figs/summaries/gA/gA_summary-1.pdf

MK_BIB		= 1
include make.tex.inc

